A Multi-perspective Analysis of Carrier-Grade NAT Deployment

As ISPs face IPv4 address scarcity they increasingly turn to network address translation (NAT) to accommodate the address needs of their customers. Recently, ISPs have moved beyond employing NATs only directly at individual customers and instead begun deploying Carrier-Grade NATs (CGNs) to apply address translation to many independent and disparate endpoints spanning physical locations, a phenomenon that so far has received little in the way of empirical assessment. In this work we present a broad and systematic study of the deployment and behavior of these middleboxes. We develop a methodology to detect the existence of hosts behind CGNs by extracting non-routable IP addresses from peer lists we obtain by crawling the BitTorrent DHT. We complement this approach with improvements to our Netalyzr troubleshooting service, enabling us to determine a range of indicators of CGN presence as well as detailed insights into key properties of CGNs. Combining the two data sources we illustrate the scope of CGN deployment on today's Internet, and report on characteristics of commonly deployed CGNs and their effect on end users.

==> Makefile <==
## Fully automated LaTeX Makefile
## (c) Bernhard Ager 2010
## Released under GPLv3 <http://www.gnu.org/licenses/gpl.txt>
##
## This is supposed to work with no (or at most a few) modifications 
## on any LaTeX source directory as a drop in.
## 
## If you have suggestions for or additions to this Makefile, feel free to
## drop me <bernhard@net.t-labs.tu-berlin.de> a mail. I am especially
## interested in further/better auto-conversion rules for picture formats.
##
## Acknowledgements go to Oliver Hohlfeld for proposing a database to track
## auto-generated pictures.
##
## Hard dependencies: GNU make, sed, grep, rm
## Soft dependencies: the tools to convert to the different formats including
## latex, pdflatex, dvips, pstopdf, eps2pdf, fig2dev, inkscape, wmf2eps, ...


## $(MAIN).tex is assumed to be the main latex file
#MAIN=$(basename $(shell grep -Fl '\documentclass' *.tex))
MAIN=paper

## $(TEXFILES) holds all LaTeX source files. Extend wildcard pattern if you
## are holding tex files in subdirectories or adjust to your needs.
TEXFILES=$(wildcard *.tex)

## $(PICTURES) and $(BIBLIOGRAPHY) try to guess the names of required 
## pictures and bib files. The matching rule is quite primitive and is
## easily confused by clutter in lines with \includegraphics or 
## \bibliography. 
PICTURES=$(shell grep -F '\includegraphics' $(TEXFILES) | \
		grep -v '%.*\\includegraphics' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfimage' $(TEXFILES) | \
		grep -v '%.*\\pgfimage' | sed 's/.*{\([^{}]*\)}.*/\1/') \
	$(shell grep -F '\pgfdeclareimage' $(TEXFILES) | \
		grep -v '%.*\\pgfdeclareimage' | sed 's/.*{\([^{}]*\)}.*/\1/')

BIBLIOGRAPHY=$(addsuffix .bib, $(shell grep -F '\bibliography{' $(TEXFILES) | \
	grep -v '%.*\\bibliography' | sed 's/.*{\([^{}]*\)}.*/\1/'))

PS_PICTURES=$(addsuffix .eps, $(PICTURES))
PDF_PICTURES=$(addsuffix .pdf, $(PICTURES))

## $(PICTURE_DB) keeps track of which pictures were actually created by
## this Makefile. In the clean target this database is used to remove them.
## You might have some manual work to do if you accidentially remove it.
PICTURE_DB = picture.db
PICTURE_DB_ADD = test -f $(PICTURE_DB) && grep -F "$@" $(PICTURE_DB) || echo "$@" >>$(PICTURE_DB)

PDFTK=/usr/bin/pdftk

## call pdflatex target if you prefer pdflatex over latex, dvips, ps2pdf
#
 all: pdflatex
# all: $(MAIN).pdf
# all: pdflatex $(MAIN).ps $(MAIN).pdf
# all: $(MAIN).pdf

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
pdflatex: $(MAIN).tex $(TEXFILES) $(PDF_PICTURES) $(BIBLIOGRAPHY)
	pdflatex $<
ifneq ($(BIBLIOGRAPHY), )
	bibtex $(MAIN) && pdflatex $< && pdflatex $<
endif
#	test -f $(PDFTK) && $(PDFTK) $(MAIN).pdf output $(MAIN)_out.pdf compress || cp $(MAIN).pdf $(MAIN)_out.pdf

.PHONY: $(MAIN).ps $(MAIN).pdf $(MAIN).dvi

$(MAIN).ps: $(MAIN).dvi
	dvips -z -P pdf -t letter -o $@ $<

$(MAIN).pdf: $(MAIN).ps
	ps2pdf -dSAFER -dNOPLATFONTS -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $< $@

## Detection of changed '\cite'ations is a PITA. Any hints welcome.
$(MAIN).dvi: $(MAIN).tex $(TEXFILES) $(PS_PICTURES) $(MAIN).bbl
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).oc
	latex $<
	grep '^\\citation' $(MAIN).aux | sort >$(MAIN).nc
	cmp $(MAIN).oc $(MAIN).nc || bibtex $(MAIN) && latex $< && latex $<

$(MAIN).bbl: $(BIBLIOGRAPHY)
	latex $(MAIN).tex
	bibtex $(MAIN).aux || true
	latex $(MAIN).tex

## unfortunately produces broken pictures, fallback to eps and eps2pdf
#%.pdf: %.dia
#	dia --export=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.dia
	dia --export=$@ $<
	$(PICTURE_DB_ADD)

%.pdf: %.fig
	fig2dev -L pdf $< $@
	$(PICTURE_DB_ADD)

%.eps: %.fig
	fig2dev -L eps $< $@
	$(PICTURE_DB_ADD)

%.eps: %.jpg
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.png
	convert $< $@
	$(PICTURE_DB_ADD)

%.pdf: %.svg
	inkscape --export-pdf=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.svg
	inkscape --export-eps=$@ $<
	$(PICTURE_DB_ADD)

%.eps: %.wmf
	wmf2eps --eps -o $@ $<
	$(PICTURE_DB_ADD)

# this rule requires the R script to plot to the correct file,
# relative to the Makefile!
%.eps: %.R
	R --no-save <$<
	test -f $@
	test $@ -nt $<

## This generic rule should be kept as the last one, so that
## native -> pdf generation takes precedence over native -> eps -> pdf
#%.pdf: %.eps
#	epstopdf --outfile=$@ $<
#	$(PICTURE_DB_ADD)

%.eps: %.pdf
	pdftops -eps $< $@
	$(PICTURE_DB_ADD)

clean:
	rm -f $(MAIN).aux $(MAIN).dvi $(MAIN).log $(MAIN).nav $(MAIN).out \
		$(MAIN).pdf $(MAIN).ps $(MAIN).snm $(MAIN).toc $(MAIN).bbl \
		$(MAIN).blg $(MAIN).oc $(MAIN).nc head.tmp body.tmp
	rm -f $(shell test -f $(PICTURE_DB) && cat $(PICTURE_DB))
	rm -f $(PICTURE_DB)

report-pictures:
	@echo $(PICTURES)

